PromptChainer: Chaining Large Language Model Prompts through Visual Programming

While LLMs can effectively help prototype single ML functionalities, many real-world applications involve complex tasks that cannot be easily handled via a single run of an LLM. Recent work has found that chaining multiple LLM runs together (with the output of one step being the input to the next) can help users accomplish these more complex tasks, and in a way that is perceived to be more transparent and controllable. However, it remains unknown what users need when authoring their own LLM chains -- a key step for lowering the barriers for non-AI-experts to prototype AI-infused applications. In this work, we explore the LLM chain authoring process. We conclude from pilot studies find that chaining requires careful scaffolding for transforming intermediate node outputs, as well as debugging the chain at multiple granularities; to help with these needs, we designed PromptChainer, an interactive interface for visually programming chains. Through case studies with four people, we show that PromptChainer supports building prototypes for a range of applications, and conclude with open questions on scaling chains to complex tasks, and supporting low-fi chain prototyping.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> backups/intro.tex <==
\section{Introduction}

Large language models (LLMs) have introduced new possibilities for prototyping with AI~\cite{yang2020re}.
Pre-trained on a large amount of unlabeled text data, models like GPT-3~\cite{brown2020language} and Jurassic-1~\cite{J1WhitePaper} encode enough information? to support \emph{in-context learning}:
they can be easily customized at run time to handle new tasks by taking in natural language instructions (also known as \emph{prompts}).
For example, a user could customize a pre-trained, general purpose LLM
to create an ad-hoc English-to-French translation engine by giving it the following
prompt string as input: \exinline{English: Hello! French: Bonjour! English: Good night French: }. An LLM would likely
continue the prompt with the French translation \exinline{Bonne nuit!}
Beyond this toy example on translation, non-ML experts have similarly used natural language prompts to achieve various ML functionalities in real-time, including code generation, question answering, creative writing, etc.~\cite{swanson2021story, mishra2021natural, brown2020language}.
Recent work on \textbf{prompt-based prototyping}~\cite{jiang2022prototype} has found that, with LLMs' fluid adaptation to natural language prompts, non-ML experts can now prototype custom ML functionality with lower effort and less time, as they bypass the otherwise necessary but expensive process of collecting data and training models upfront~\cite{jiang2022prototype,bommasani2021opportunities}.

Despite the demonstrated versatility of LLMs, many real-world applications involve complex or multi-step tasks, which often cannot be effectively handled via a single run of an LLM.
For example, a music chatbot may require an AI to generate different kinds of responses depending on the query types, \eg asking for a song versus requesting information about an artist. 
%For example, a music chatbot may require an AI to handle branching logic, by first determining the type of user query (\eg asking for a song, asking about artists, asking about albums, etc.), before generating a response based on the query category. \ellen{I feel like calling this branching logic with an order implies that a 2-step chain is necessary, even though this problem can also be thought of as 1 single step where we ask more of the model, i.e. with few shot examples that span the different types of queries. Maybe we could say 'a music chatbot may require an AI to generate a different kind of response depending on the type of query, i.e. asking for a song versus requesting information about an artist. Due to the complexity of such tasks, designers and developers may struggle...}
As a result, designers and developers may struggle to prototype realistic applications with a single LLM. 
In response, Wu \etal~\cite{wu2021ai} proposed \emph{Chaining} multiple LLM runs together, \ie decomposing an overarching task into a series of highly targeted sub-tasks, mapping each to a distinct LLM step, and using the output from one step as an input to the next.
%For example, as we will see later in Figure~\ref{fig:example}, a chain for the aforementioned music chatbot may involve \emph{LLM classifiers} on user intents, as well as specialized \emph{LLM response generators} per intent.
Through user studies, Wu \etal observed that Chaining successfully raises the ceiling of what tasks users can meaningfully accomplish using LLM chains, while simultaneously increasing the transparency and controllability of the AI system. %in a transparent and controllable manner, and envisioned that chaining can further help prototype more complex flows of AI-infused applications.

While this past work examined the utility of LLM chains, and how people can \emph{use} these chains, it remains an open question of how to support users in \emph{authoring} their own LLM chains. % \carrie{need a sentence justifying why authoring is important (beyond using)}
%Akin to software design~\cite{pressman2005software}, c
For example, chain authoring requires users to not only prompt within each individual LLM step, but also design the overarching task decomposition, which includes defining the relationships and interactions between LLM steps.
Whereas Wu \etal's work provided predefined chain structures for participants to use, explicit support for chain authoring requires targeted tooling to help designers and developers apply chaining to their own applications and prototypes, akin to end-user programming~\cite{Burnett2004EnduserSE, burnett2010end}.
\ellen{what is end-user programming? I'm a little confused if that means writing code or not - perhaps the citation would help clarify it.} 
\sherry{for Ellen - it's a programming paradigm widely accepted and studied in HCI. End users do not code, but define ``APIs'' or examples they want a software to handle, and these tools help translate APIs into actual programs. You can delete it afterwards!}

In this work, we ask: \textbf{How can we help non-ML experts \emph{author} LLM chains for their own tasks?} 
We distill unique challenges in LLM Chain authoring through formative studies, and propose an interface to that supports interactively construction and interation on Chains.
The interface offers three primary scaffolding in response to the challenges:
(1) it automatically parsesurface the node structures LLM prompts into Chaining APIs, to ease the mental demand on connecting local LLM implementations with global Chain structures;
such that users can iterate on their prompts without unconsciously breaking the chain; 
(2) it 


The interface automatically surfaces the node structures (\ie required inputs and generated outputs) based on the underlying LLM prompts, such that users can iterate on their prompts without unconsciously breaking the chain.
By defining a list of predefined helper nodes, we help evaluate LLM outputs and guard against LLM errors, provide scaffolding on typical data transformation (\eg parse a string into a list of ideas).
We further provide an example gallery with typical prompting formats, which implicitly encourages end users prompt their LLMs in ways that the helper nodes can parse.



The interface automatically surfaces the node structures (\ie required inputs and generated outputs) based on the underlying LLM prompts, such that users can iterate on their prompts without unconsciously breaking the chain.
By defining a list of predefined helper nodes, we help evaluate LLM outputs and guard against LLM errors, provide scaffolding on typical data transformation (\eg parse a string into a list of ideas).
We further provide an example gallery with typical prompting formats, which implicitly encourages end users prompt their LLMs in ways that the helper nodes can parse.



Through a series of formative studies, we distill unique challenges 

three unique challenges in LLM Chain authoring:
(1) With LLMs taking unstructured prompts, they lack explicit ``function signatures,'' making LLM prompting disconnected from the overarching chain construction; %, and closely bridging the two level of implementation is important.
(2) With LLM versatility, fully unassisted prompts can lead to outputs in arbitrary formats, making it nontrivial to transform intermediate data points;
(3) With LLMs being black-boxes, their potentially low-quality, counter-intuitive, or even unsafe outputs can make LLM Chains more prone to cascading errors.

\mike{Maybe this to streamline (a fair bit is cut out): 
In this work, we examine the user experience of \emph{authoring} LLM chains. Specifically, we conducted case studies with four designers and developers, in which they proposed their own application ideas, and designed and built chains for it.
Our qualitative analysis of these case studies reveals interesting patterns on how users build and debug chains: (1) users build chains not only for addressing LLM limitations (as expected), but also for making the prototype extensible;
(2) users perform iterative chain construction, sometimes chaining half-baked or even written prompts to illustrate the high level logic;
(3) the interactions between multiple LLM prompts can be complex, requiring both local and global debugging of prompts (\eg a downstream prompt may be affected by the design of an upstream prompt, requiring debugging of both).}

%, making extensive debugging necessary.


%Through a series of formative studies, we found that authoring LLM chains requires close connection between the underlying prompting implementation and the exposed data structure per LLM module, careful scaffolding for tracking and transforming intermediate data points, as well as debugging the chain at multiple granularities. 



\begin{figure}[t]
\centering
%\begin{subfigure}{1\textwidth}\centering

\includegraphics[trim={0 36cm 7.5cm 0cm}, clip, width=1\columnwidth]{figures/ui.pdf}
\vspace{-20pt}
\caption{
The chain authoring interface. 
(A) The \emph{Chain View} visualizes the chain structure in the form of a node-link diagram, and allows users to edit the chain by adding, removing, or reconnecting nodes.
(B) The \emph{Node Editing Panel} supports implementing, improving, and testing each individual node, \eg editing prompts for LLM nodes.
Besides executing and debugging individual nodes, the interface also supports running the chain end-to-end (C). 
(D) We define a wide list of node types, which users can select from the node library.
}
%\vspace{-10pt}
\label{fig:ui}
\end{figure}

\carrie{could probably shorten this whole section to just 2-3 sentences since redundant with rest of paper: 
In response, we propose an interface that supports users to interactively construct and improve the LLM Chains in the form of node-link diagrams, as shown in Figure~\ref{fig:ui}.
The interface automatically surfaces the node structures (\ie required inputs and generated outputs) based on the underlying LLM prompts, such that users can iterate on their prompts without unconsciously breaking the chain.
By defining a list of predefined helper nodes, we help evaluate LLM outputs and guard against LLM errors, provide scaffolding on typical data transformation (\eg parse a string into a list of ideas).
We further provide an example gallery with typical prompting formats, which implicitly encourages end users prompt their LLMs in ways that the helper nodes can parse.

To evaluate the interface, we conducted case studies with four designers and developers, in which they proposed their own application ideas, and designed and built chains for it.
We show that our interface broadly supports building prototypes for various realistic tasks (\eg building chatbots, writing assistants, etc.).
In particular, our debugging mechanisms effectively helped users locate seemingly global errors to local causes, and our helper functions also alleviated the overhead on transforming intermediate data points, and end users used three times as much predefined transformation functions compared to customized ones.}
Though the study is still preliminary, our qualitative analyses reveal interesting patterns on how users build and debug chains: (1) users build chains not only for addressing LLM limitations (as we originally expected), but also for making the prototype extensible;
(2) users perform iterative chain construction, sometimes chaining half-backed or even not-yet-prompted LLMs to illustrate the high level logic;
(3) the interactions between multiple LLMs in a chain impact how users debug and implement each of them.

\mike{The interesting tidbits here seem to be: 1) friction for exploring multiple alternatives, 2) preserving global context and coherence, and 3) scaling. We may want to tighten to just 3 challenges}
We also observed some challenges in chain authoring: %While the chains in our study had moderate chain lengths, we began to observe emerging user challenges around: 
applying chain execution to multiple inputs, scaling to complex chains with large numbers of nodes or branches, and preserving global context and coherence. Finally, users who invested time constructing local prompts for each LLM step were less inclined to explore alternative global chain structures. This raises the question of how to encourage low-fi prototyping of \emph{multiple} alternative chain structures: in other words, what is the ``sweet spot'' of prompting, that is lightweight to construct while being sufficient for feasibility testing?   %to start to see some challenges on building more complex chains. 
%First, our users came with fully designed chains, it remains unclear how would users switch between gradual chain expansion and prompting, if the task is too complex to decompose at once. 
%Second, as the chain grow more complicated, they would also require advanced mechanisms for context-preservation and modular debugging.
%Third, we also notice some users started with fairly sophisticated LLM prompts, which may make them more inclined to make \emph{local} iterations within LLM prompts, without altering the \emph{global} chain structure (which may require prompting from scratch).
%This raises the challenge of encouraging low-fi prototyping with LLMs: what is the ``sweet spot'' of prompting, that is lightweight enough while being sufficient for feasibility testing?
In the future, we plan to explore these open questions through longer-term studies, where we observe users build and interact with complex chains over time.


==> backups/requirement.tex <==
\subsection{Formative Study Formats}
To inform the design of our tools, we conducted participatory design sessions with three engineers, and iteratively refined the interface with two UX designers through a three-month period. 

Through a three-month design iteration, 

To inform this research, we conducted the following three sets of formative studies to distill user needs and design requirements for chain authoring.

\begin{itemize}[leftmargin=1.2em,labelwidth=*,align=left, nosep]
\item \textbf{Exploratory study}
We observed a wide range of industry practitioners (20 UX designers, front-end engineers, and data analysts) to further distill user needs when refining and modifying chaining structures.
Following Wu \etal~\cite{wu2021ai}'s study design, we provided them with a pre-defined chain (built either for brainstorming flashcards or rewriting peer reviews), and asked them to \emph{modify} those chains to improve them. %asked them to get familiar with the default by using the chain on the given task. 
%We then asked the participants to \emph{modify} the defaults, to observe their needs and actions when refining the chaining structures. 

\item \textbf{Design Sessions.}
We invited another three engineers each for a 30-45 minute design discussion.
They were not part of the exploratory study, but were particularly interested in chaining and have manually built chains on their own.
In the sessions, we guided the engineers to reflect on their own experiences building chains, with some seeding questions on their processes (\quoteinline{What was your starting point for creating chains?}) or the challenges they faced (\quoteinline{What help did you need for connecting multiple LLM steps?}).

\item \textbf{Long term iterations.}
Finally, we worked closely with two UX designers (one from the design session) over the course of three months, to iteratively test our designs on four of their example chains.
These examples, summarized in Appendix~\ref{appendix:pilot_chains}, cover a wide range of use cases, including reading assistant (iteratively summarizing long essays), instant message handler (determining if an incoming message deserves immediate attention), etc.
We used these test cases to plan out the initial required functionalities, and the engineers recreated their chains for several rounds in the iterations, reporting back their pain points throughout.
\end{itemize}

\subsection{Design Requirements}








\begin{enumerate}[itemsep=20pt,leftmargin=0em,labelwidth=-2em,align=left, nosep,label=R.\arabic*]
\setlength\itemsep{0.5em}
%[nosep,labelwidth=*,leftmargin=1.8em,align=left,label=R.\arabic*]
\item \label{require:connect}
\textbf{

Closely connect low-level LLM prompts and high-level chain structure.}
Since LLMs modules are ``implemented'' with unstructured natural language prompts, they lack explicit functional signatures as in typical programming environments.
In the design sessions, our engineers mentioned that it is mentally demanding to switch context between building chains and prompting, \eg having to double check whether the number and ordering of input text is compatible to a new prompt version.  

\item \label{require:model_capability}
\textbf{Provide scaffolding on LLM functionalities and data transformation.}
Another challenge brought by LLMs' unstructured nature is the unclear LLM capability and the nontrivial data transformation involved. 
In design sessions, we saw users prompting LLMs to generate a wide range of text structure, ranging from stringfied JSON and array, to bullet list, to descriptive text.
Such diversity renders the data transformation need unpredictable, and forces each chain author to write a large amount of data processing functions accordingly (\eg parse and extract a particular field from a generated JSON text).
However, underneath their diverse prompt structure, their use of LLMs all broadly fall under the three categories Wu \etal identified, \ie to use the LLM for a list of ideas and examples (\emph{Ideation}), to assign inputs to certain categories for branching logic or validation (\emph{classification}), and to gather certain information from the input (\emph{Info. Extraction}).
Some minor rewrites on their prompts are usually enough for unifying the data parser needed, without breaking the desired LLM functionality.
For example, when generating a list of country artists, instead of prompting LLMs to output descriptive sentence \quoteinline{there are Garth Brooks, George Strait, and Dolly Parton}, generating a numbered list of \quoteinline{1) Garth Brooks 2) George Strait 2) Dolly Parton} would make the output easily parsable regular expressions on numbers.

In contrast, our exploratory study participants did not face such burden, as they primarily relied on the aforementioned primitive operations, which provided strictly structured prompt formats for all the typical LLM functionalities in a chain. 
These operations served three goals:
(1) they capitalized the possible functionalities in the otherwise seemingly all-encompassing model;
(2) they onboarded the participants to prompting by providing feasible starting points via templates;
(3) they enable easy data transformation, as their prompt templates force the LLM output to follow certain predictable patterns that can be easily parsed with predefined post-processing functions (like the artist ideation example above).
%For example, in \emph{Ideation}, their prompt templates ensures LLMs to generate lists in the form of \exinline{1) San Diego 2) San Francisco}), which they can later split by regular expressions on numbers.
Though we decided not to use strict templates (which, participants found too constrained and limited in generalizability), we conclude that chain authors similarly need some soft scaffolding for core LLM functionalities, their typical prompting strategies, and associated data processors.
\item \label{require:debugging}
\textbf{Enable debugging at multiple levels of granularity.}
LLMs are trained in a black-box manner. 
They generate text based on standard sampling likelihood that are not necessarily aligned with human intuitions~\cite{holtzman2019curious}, nor are they guaranteed to generate fair or ethical outputs~\cite{talat2021word, jiang2021delphi}.
As such, multiple formative study participants expressed their concerns about whether chaining would cause cascading errors.
In response, we require our interface to provide evaluation and filtering scaffoldings around LLM outputs, which should guardrail the quality of each LLM output.

Besides the automated filtering, Wu \etal~\cite{wu2021ai} also observed that exposing intermediate data points to users effectively help them interactively debug the chain.
Following their observations, we similarly design our interface to allow for debugging at different granularities:
(1) \emph{unit testing} each individual LLM node independent of others;
(2) \emph{Breakpoint debugging} by observing and fixing stepwise, intermediate outputs, to local global errors to local causes; 
(3) \emph{End-to-end chain assessment} by running the entire chain, and use the final output as immediate feedback on whether an intermediate fix was successful globally.
\end{enumerate}


==> tables/case_table_for_poster.tex <==
%\begin{table*}[h]
\renewcommand{\arraystretch}{0.8}
\fontsize{7.5}{8}\selectfont
\begin{tabular}{r | l | l}
\toprule
\textbf{Node Type} & \textbf{Description} & \textbf{Example in Figure} \\

\midrule\midrule
\multicolumn{3}{l}{\textbf{LLM Nodes}: Core implementations of LLM prompts, for either generic use or filtering.}\\
\midrule
Generic LLM 
    & Use the LLM output directly as the node output. 
    & \textcircle{4} \textcircle{6} \textcircle{9} \\
\midrule
LLM Classifier 
    & Use LLM output to filter and branch out inputs. 
    & \textcircle{2} \textcircle{3} \\


\midrule\midrule
\multicolumn{3}{l}{\textbf{Helper Nodes}: Common data transformation and evaluation needs.}\\
\midrule
Evaluation 
    & Re-rank LLM outputs by customized criteria, \eg politeness.
    & \textcircle{10} Toxicity classifier\\
\midrule
Processing 
    & Pre-implemented JS functions for typical data transformation. %(between a single string and a list of strings).
    & \textcircle{5} Split by number\\
\midrule
Generic JS 
    & User-defined JS functions for further customization.
    & \textcircle{8} Format the query\\

\midrule\midrule
\multicolumn{3}{l}{\textbf{Communication Nodes}: Exchange data with the external world (e.g. external API calls).}\\
\midrule
Data Input 
    & Define the input to a chain.
    & \textcircle{1}\\
\midrule
User Action 
    & Enables end user editing on intermediate data points.
    & \\
\midrule
API Call 
    & Connect external, professional services with LLMs.
    & \textcircle{6} Call YouTube API\\
\bottomrule
\end{tabular}
\vspace{-10pt}
\caption{A summary of node types, including the core \textbf{LLM nodes}, \textbf{helper nodes} for data transformation and evaluation, and \textbf{communication nodes} for exchanging LLM data with external users or services.}
\vspace{-5pt}
\Description{The table summarizes all the node types in detail. It includes the core LLM nodes, helper nodes for data transformation and evaluation, and communication nodes for exchanging LLM data with external users or services.}
\label{table:node_types}

%\vspace{-10pt}
%\end{table*}


==> tables/case_table_for_poster_v2.tex <==
%\begin{table*}[h]
\renewcommand{\arraystretch}{0.8}
\fontsize{7.5}{8}\selectfont
\begin{tabular}{p{0.005\linewidth} l | l | l}
\toprule
\multicolumn{2}{l}{\textbf{Node Type}} & \textbf{Description} & \textbf{Example in case} \\

\midrule\midrule
\multirow{2}{*}{\rotatebox[origin=c]{90}{LLM}}
& Generic LLM 
    & Use the LLM output directly as the node output. 
    & \textcircle{4} \textcircle{6} \textcircle{9} \\
\cmidrule(lr){2-4}
& LLM Classifier 
    & Use LLM output to filter and branch out inputs. 
    & \textcircle{2} \textcircle{3} \\


\midrule\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Helper}} 
& Evaluation 
    & Re-rank LLM outputs by human-designed criteria, \eg politeness.
    & \textcircle{10} Toxicity classifier\\
\cmidrule(lr){2-4}
& Processing 
    & Pre-implemented JS functions for typical data transformation. %(between a single string and a list of strings).
    & \textcircle{5} Split by number\\
\cmidrule(lr){2-4}
& Generic JS 
    & User-defined JS functions for further customization.
    & \textcircle{8} Format the query\\

\midrule\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Comm.}} 
& Data Input 
    & Define the input to a chain.
    & \textcircle{1}\\
\cmidrule(lr){2-4}
& User Action 
    & Enables external (end user) editing on intermediate data points.
    & \\
\cmidrule(lr){2-4}
& API Call 
    & Call external functions to connect professional services with LLMs.
    & \textcircle{6} Call YouTube API\\
\bottomrule
\end{tabular}
\vspace{-10pt}
\caption{A summary of node types, including the core \textbf{LLM nodes}, \textbf{helper nodes} for data transformation and evaluation, and \textbf{communication nodes} for exchanging LLM data with external users or services.}
\vspace{-5pt}
\Description{The table summarizes all the node types in detail. It includes the core LLM nodes, helper nodes for data transformation and evaluation, and communication nodes for exchanging LLM data with external users or services.}
\label{table:node_types}

%\vspace{-10pt}
%\end{table*}


==> todo.tex <==
-- PRIMARY CHAIN FUNCTION --
| # chains 11
| primary use [('classify', 3, 27.3), ('extract', 4, 36.4), ('ideate', 4, 36.4)]
| classify    	|  ['classify', 'generate', 'generate']
| extract    	|  ['rewrite', 'rewrite']
| classify    	|  ['classify', 'generate', 'generate', 'generate']
| ideate    	|  ['ideate', 'ideate']
| ideate    	|  ['ideate', 'ideate', 'classify', 'ideate']
| extract    	|  ['extract', 'classify']
| ideate    	|  ['ideate', 'ideate']
| classify    	|  ['classify', 'classify', 'rewrite']
| extract    	|  ['generate', 'extract', 'generate', 'generate', 'rewrite', 'rewrite', 'classify', 'classify']
| ideate    	|  ['ideate', 'rewrite']
| extract    	|  ['extract', 'classify', 'extract', 'extract', 'classify', 'rewrite']

-- CHAIN SIZE --
| # nodes included:  MEAN=5.55, STD=2.19

-- NODE TYPE DISTRIBUTION --
| %llm
	 MEAN=0.65, STD=0.27
| %helper_default
	 MEAN=0.23, STD=0.21
| %helper_custom
	 MEAN=0.12, STD=0.14

-- NODE TYPE DISTRIBUTION --

| llm (N=38)
| [('classify', 10, 26.3), ('generate', 8, 21.1), ('rewrite', 7, 18.4), ('ideate', 8, 21.1), ('extract', 5, 13.2)]

| helper_default (N=14)
| [('split', 7, 50.0), ('join', 4, 28.6), ('jshelper', 2, 14.3), ('useraction', 1, 7.1)]

| helper_custom (N=9)
| [('parse_llm_multiple_output', 1, 11.1), ('format_llm_output', 6, 66.7), ('pair_llm_input_output', 2, 22.2)]

